A Two-Part Controller Synthesis Approach for Nonlinear Stochastic Systems Perturbed by L\'evy Noise Using Renewal Theory and HJB-Based Impulse Control

We are motivated by the lack of discussion surrounding methodological control design procedures for nonlinear shot and L\'evy noise stochastic systems to propose a hierarchical controller synthesis method with two parts. The first part is a primitive pattern-learning component which recognizes specific state sequences and stores in memory the corresponding control action that needs to be taken when the sequence has occurred. The second part is a modulation control component which computes the optimal control action for a pattern when it has occurred for the first time. Throughout our presentation of both components, we provide a self-contained discussion of theoretical concepts from Poisson processes theory, renewal theory, and impulse control, all of which are necessary as background. We demonstrate application of this controller to the simplified, concrete case studies of fault-tolerance and vehicle congestion control.

==> arxiv_sections/pattern_occurrence.tex <==
% \violet{FIX NOTATION:\\
% \begin{example}
%     We are tossing a coin that lands heads with probability $p$, and tails with probability $q = 1 - p$. Compute the expected number of coin tosses it takes to get the sequence $HHT$.

%     Let $E$ be the event where we get the desired sequence. Condition on whether we get a heads or a tails on the first toss.
%     \begin{align*}
%         \Ebb[E] &= \Ebb[E|H]\Pbb(H) + \Ebb[E|T]\Pbb(T) = \Ebb[E|H]p + \Ebb[E|T]q
%     \end{align*}
%     Note that $\Ebb[E|T] = 1 + \Ebb[E]$ since we want a heads in the first toss in order to begin counting for our sequence, but we've already tossed the coin once, so we add a one.

%     Now $\Ebb[E|H]$ can be further conditioned on whether we get a heads or a tails on the second toss.
%     \begin{align*}
%         \Ebb[E|H] &= \Ebb[A|HH]\Pbb(H|H) + \Ebb[A|HT]\Pbb(T|H) = \Ebb[A|HH]p + \Ebb[A|HT]q
%     \end{align*}
%     By similar reasoning as above, we have that $\Ebb[A|HT] = 2 + \Ebb[E]$. Also, $\Ebb[A|HH] = 2 + \frac{1}{q}$, since now that we have the first two heads, all we have to wait is for the first tail to land, and the number of tosses required for such is a geometric random variable with parameter $q$.

%     Hence
%     \begin{align*}
%         \Ebb[E|H] &= (2 + \frac{1}{q})p + (2 + \Ebb[E])q = 2p + \frac{p}{q} + 2q + q\Ebb[E] = 2 + \frac{p}{q} + q\Ebb[E]
%     \end{align*}
%     Substituting this into our original expression for $\Ebb[E]$, we get:
%     \begin{align*}
%         &\Ebb[E] = (2 + \frac{p}{q} + q\Ebb[E])p + (1 + \Ebb[E])q = 2p + \frac{p^2}{q} + qp\Ebb[E] + q + q\Ebb[E]\\
%         \Longrightarrow \ &(1 - qp - q)\Ebb[E] = 2p^2 + \frac{p^2}{q} + 2pq + q\\
%         \Longrightarrow \ &p^2\Ebb[E] = 2p^2 + \frac{p^2}{q} + 2pq + q\\
%     \end{align*}
%     Now we get:
%     \begin{align*}
%         \Ebb[E] = \frac{2p^2q + p^2 + 2q^2p + q^2}{p^2q}
%     \end{align*}
%     Note that the numerator of this expression can be simplified as follows:
%     \begin{align*}
%         &2p^2q + p^2 + 2q^2p + q^2 = 2p^2(1 - p) + p^2 + 2(1 - p)^2p + (1 - p)^2 = 1
%     \end{align*}

%     So our final answer is $\frac{1}{p^2q}$. We can visualize this with the figure~\fig{cond_seq_pattern}. If we were to obtain the sequence immediately since we start tossing the coin, the endpoint of the trajectory we desire would be as circled.

%     % We can compute the expected value of obtaining our desired sequence $HHT$ from every point. First we consider the following trajectory
%     \begin{figure}
%         \begin{center}
%             \includegraphics[width=0.3\columnwidth]{../figures/126figs-5.pdf}
%         \end{center}
%         \caption{Random walk-like representation of coin toss trials, where the horizontal axis marks the number of tosses made, and the walk travels up one unit if the coin lands heads, down one unit otherwise.}
%         \label{fig:cond_seq_pattern}
%     \end{figure} 
% \end{example}
% }

%%%%% CANNOT PUT THIS HERE BECAUSE THE COMBINED THEOREM DEALS WITH RENEWAL REWARD PROCESSES TOO
% \subsection{Important Theorems for Renewal Processes}\label{sec:renewal_theorems}
% \import{arxiv_sections/}{renewal_theorems_combined.tex}

With the renewal theory background established, we now consider the general problem of \textit{pattern occurrence}. We first discuss a motivational example before describing a more general result. 

\begin{example}
    Suppose that we are observing a sequence of iid binary random variables $X_1, X_2, \cdots$, each with distribution
    \begin{align*}
        X_i = \begin{cases}
            1 &\text{ with probability } \ p\\
            0 &\text{ with probability } \ q := 1-p
        \end{cases}
    \end{align*}
    Two common problems of interest for this setup are 1) the expected time, i.e. number of random variables observed in the sequence, it takes to see either a string of $n$ ones or $m$ zeros, and 2) the probability of observing $n$ ones before $m$ zeros. 

    We address the first part of the first problem: what is the expected time it takes to observe a string of $n$ ones? Denote $\Ebb[(k,1) | (j,1)]$ for $0\leq j\leq k$ to be the expected time it takes to observe a string of $k$ ones given we have already observed a string of $j$ ones. Then the conditional expectation of interest is $\Ebb[(n,1)] := \Ebb[(n,1) | (0,1)]$. We can set up a series of $n$ equations with $n$ conditional expectations as the unknowns:
    \begin{align*}
        &\Ebb[(n,1)] = p(1 + \Ebb[(n,1)|(1,1)]) + q(1 + \Ebb[(n,1)]) = 1 + p\Ebb[(n,1)|(1,1)] + q\Ebb[(n,1)]\\
        &\Ebb[(n,1) | (k,1)] = 1 + p\Ebb[(n,1) | (k+1,1)] + q\Ebb[(n,1)], \ \ 1\leq k\leq n-2\\
        &\Ebb[(n,1) | (n-1,1)] = 1 + q\Ebb[(n,1)]
    \end{align*}
    Iteratively substituting the equations backwards until $k=1$ yields:
    \begin{align*}
         \Ebb[(n,1) | (1,1)] = \sum\limits_{j=0}^{n-2}p^j + q\sum\limits_{j=0}^{n-2}p^j \Ebb[(n,1)]
    \end{align*}
    and ultimately:
    \begin{align}\label{eq:motive_success_time}
        \Ebb[(n,1)] = \sum\limits_{j=1}^n \frac{1}{p^j}
    \end{align}

    The second part of the first problem is solved similarly, with the unknown conditional expectations denoted $\Ebb[(k,0) | (j,0)]$ for $0\leq j\leq k$ instead. With the same rote computation, we get
    \begin{align}\label{eq:motive_failure_time}
        \Ebb[(m,0)] = \sum\limits_{j=1}^m \frac{1}{q^j}
    \end{align}
    % Note that these expressions match exactly what we would have obtained using the formula for patterns with overlaps in the pattern occurrence theorem. 

    Now we are ready to address the second problem. Let $E$ be the event that we get $n$ consecutive ones before $m$ consecutive zeros. Let $S$ denote the event that a $1$ is first observed in the sequence, and $F$ denote the event that a $0$ occurred instead. By conditional probabilities, we get $\Pbb(E) = \Pbb(E|S)*p + \Pbb(E|F)*q$, where
    \begin{align*}
        \Pbb(E|S) = p^{n - 1} + (1 - p^{n - 1})\Pbb(E|F), \qquad \Pbb(E|F) = (1 - q^{m - 1})\Pbb(E|S)
    \end{align*}
    % For details on how these equations were derived, we refer the reader to~\cite{han21book}.
    and solving the system yields
    \begin{align}\label{eq:motive_prob}
        \Pbb(E) &= \Pbb(E|S)*p + \Pbb(E|F)*q = \frac{q^{m - 1}(1 - p^n)}{p^{n - 1} + q^{m - 1} - p^{n - 1}q^{m - 1}}
    \end{align}
\end{example}

The discussion of this simple example segways naturally to more complicated pattern sequences and broader probability distributions of $X_i$, i.e. those that take more than two values. The next theorem provides a result for when there is dependence among the values of $X_i$.

\begin{definition}[Pattern Overlap]
    For a renewal process $X_1, X_2,\cdots$ taking values $x_1, x_2, \cdots$ from a certain probability distribution, we say that a pattern $(x_{(1)}, x_{(2)}, \cdots, x_{(m)})$ has an overlap of size $k < m$ if
    \begin{align*}
        k := \max\{\ell < m | (x_1, \cdots, x_{\ell}) = (x_{m-\ell+1}, \cdots, x_m)\}
    \end{align*}
    That is, $k$ is the largest value such that the first $k$ elements are identical to the last $k$ elements.
    % A pattern $(x_1,\cdots, x_m)$ has overlap of size $k$ if:
    % \begin{align*}
    %     k = \max\{j < m : (x_{m-j+1},\cdots,x_m) = (x_1, \cdots, x_j)\}
    % \end{align*}
    % That is, there exists a size $j$ subsequence of the pattern at the end which matches another size $j$ subsequence of the pattern at the front. 
\end{definition}

\begin{theorem}[Pattern Occurrence for Discrete-State Markov Chain]\label{thm:pattern_occurrence_mc}
    Let $X_1, X_2,\cdots$ denote a sequence of random variables taking values from a discrete-state Markov Chain with transition probability matrix $P := \{P_{ij}\}$ and stationary distribution $\{\pi_k\}$. Let $T$ denote the next time the pattern $(x_1, \cdots, x_m)$ occurs after its first occurrence. 
    % In this problem, we are interested in the expected value of $T$. Within the specific context of the pattern occurrence problem, we refer to a ``renewal'' as the event when the pattern string $(x_1, \cdots, x_m)$ repeats itself. Hence, the interarrival times of such a renewal process are distributed in the same manner as $T$.
    Then:
    \begin{itemize}
        \item When the pattern $(x_1,\cdots,x_m)$ does not contain any overlaps. then the expected time $T$ in between consecutive observations of the pattern is given by
        \begin{align}\label{eq:T_no_overlap_mc}
            \Ebb[T|X_0 = x_0] = \frac{1}{\pi_{x_1}\prod\limits_{i=1}^{m-1} P_{x_i,x_{i+1}}} + \mu(x_0,x_1) - \mu(x_m,x_1)
        \end{align}
        where $\mu(x,y)$ denotes the mean time it takes to reach state $y$ in the Markov chain from state $x$.

        \item When the pattern $(x_1,\cdots,x_m)$ has an overlap $(x_1,\cdots,x_k)$ of size $k$, and $(x_1,\cdots,x_k)$ itself does not contain any overlaps, then the expected time $T$ in between consecutive observations is given by
        \begin{align}\label{eq:T_overlap_mc}
            \Ebb[T|X_0 = x_0] = \frac{1}{\pi_{x_1}\prod\limits_{i=1}^{m-1} P_{x_i,x_{i+1}}} + \frac{1}{\pi_{x_1}\prod\limits_{i=1}^{k-1} P_{x_i,x_{i+1}}} + \mu(x_0,x_1) - \mu(x_m,x_1)
        \end{align}
    \end{itemize}
\end{theorem}

\begin{example}[\thm{pattern_occurrence_mc} for iid Sequence]\label{ex:pattern_occurrence_iid}
    We can specialize the results of~\thm{pattern_occurrence_mc} to the case where the random variables $X_i$ are iid. Let $X_1, X_2,\cdots$ denote a sequence of iid random variables taking on values from a discrete, finite set $\Xcal$. Denote $p_k := \Pbb(X_i= k)$ for all $i$, and let $T$ denote the next time the pattern $(x_1, \cdots, x_m)$ occurs after its first occurrence. Then:
    \begin{itemize}
        \item When the pattern $(x_1,\cdots,x_m)$ does not contain any overlaps. then the expected time $T$ in between consecutive observations of the pattern is given by
        \begin{align}\label{eq:T_no_overlap_iid}
            \Ebb[T] = \frac{1}{\prod\limits_{i=1}^m p_{x_i}}
        \end{align}

        \item When the pattern $(x_1,\cdots,x_m)$ has an overlap $(x_1,\cdots,x_k)$ of size $k$, and $(x_1,\cdots,x_k)$ itself does not contain any overlaps, then the expected time $T$ in between consecutive observations is given by
        \begin{align}\label{eq:T_overlap_iid}
            \Ebb[T] = \frac{1}{\prod\limits_{i=1}^m p_i} + \frac{1}{\prod\limits_{i=1}^{k} p_i}
        \end{align}
    \end{itemize}
\end{example}

\begin{remark}
    Some of the standard references in renewal theory~\cite{ross96book,ross06book,ross10book} also provide some discussion on the pattern-occurrence problem from renewal theory, but often only present the iid case of~\exa{pattern_occurrence_iid}. In~\thm{pattern_occurrence_mc}, we extended this result to include a possible dependence structure for its relevance to the specific fault-tolerance and congestion control case studies we investigate later in~\sec{case_studies}. While a rough sketch of the proof for the iid case~\exa{pattern_occurrence_iid} can be found in~\cite{ross96book}, we provide a more detailed derivation of the formulas in our work~\cite{han21book}. The proof to~\thm{pattern_occurrence_mc} can also be found in~\cite{han21book}.
\end{remark}

% The extended version of the problem, which is a problem of interest in more general settings of renewal processes, looks into computing the probability of observing a specific pattern first among a predetermined set of patterns we wish to observe. We investigate the more general problem after addressing this simpler coin tossing problem.
Furthermore, we can address the question of comparing multiple different patterns at once. Let $\{A_1, \cdots, A_M\}$ for $M\in\Nbb^{+}$ be $M$ different patterns of interest, and let $T_{A_i}$ denote the time it takes to observe pattern $A_i$. Denote $T_{\text{min}} := \min\{T_{A_1}, \cdots, T_{A_M}\}$ and denote $P_i$ to be the probability of observing pattern $A_i$ first at time $T_{\text{min}}$. We further denote $T_{A_i|A_j}$ to be the additional time it takes to observe the pattern $A_i$ after $A_j$ has been observed. We are interested in computing the $P_i$ and $\Ebb[T_{\text{min}}]$. 

We further denote $T_{A_i|A_j}$ to be the additional time it takes to observe sequence $A_i$ given that we've already observed $A_j$, for all $i\neq j$. Since all the patterns $\{A_1, \cdots, A_M\}$ are known, both $\Ebb[T_{A_i}]$ and $\Ebb[T_{A_i|A_j}]$ can be computed using either~\thm{pattern_occurrence_mc} or~\exa{pattern_occurrence_iid}. We can then derive a system of equations with these variables as follows:
\begin{align*}
    \Ebb[T_{A_k}] &= \Ebb[T_{\text{min}}] + \Ebb[T_{A_k}-T_{\text{min}}] = \Ebb[T_{\text{min}}] + \sum\limits_{j\neq k}\Ebb[T_{A_k|A_j}]P_j + 0\cdot P_k
\end{align*}
which, combined with the constraint that $P_M := 1 - \sum_{i<M}P_i$ yields $M$ linear equations with $M$ unknowns $P_1, \cdots, P_{M-1}, \Ebb[T_{\text{min}}]$. For the case where $M=2$, we obtain the explicit formula:
\begin{align}\label{eq:min_time_first_prob}
    P_1 &= \frac{\Ebb[T_{A_2}] + \Ebb[T_{A_1|A_2}] - \Ebb[T_{A_1}]}{\Ebb[T_{A_2|A_1}] + \Ebb[T_{A_1|A_2}]},\qquad \Ebb[T_{\text{min}}] = \Ebb[T_{A_2}] - \Ebb[T_{A_2|A_1}]P_1
\end{align}

Note that, when we return to the motivating example and compute the expected times to obtain $n$ consecutive ones and $m$ consecutive zeros, respectively, using~\exa{pattern_occurrence_iid}, we obtain the exact same formulas as in~\eqn{motive_success_time} and~\eqn{motive_failure_time}, derived using the brute-force strategy. Substituting these results into~\eqn{min_time_first_prob} yields the original result~\eqn{motive_prob}.

% \begin{proof}
%     We isolate the analysis to two specific cases:
%     \begin{itemize}
%         \item \textit{\textbf{Case 1: there is no pattern overlap.}} In this case, it is intuitive that the occurrence time $T$ can be treated as a geometric random variable. Hence,
%         \begin{align}\label{eq:T_no_overlap}
%             \Ebb[T] = \frac{1}{\prod\limits_{i=1}^m p_{x_i}}
%         \end{align} 
%         since $\prod_{i=1}^m p_{x_i}$ is the probability of observing exactly the sequence $(x_1,\cdots, x_m)$. 
%         For a more comprehensive derivation of this formula, note that $T > n+m$ iff the pattern does not occur for the first $n$ values, and the next $m$ values are $(x_1,\cdots, x_m)$. That is:
%         \begin{align*}
%             \{T>n+m\} \Longleftrightarrow \{T>n \text{ and } (X_{n+1},\cdots,X_{n+m}) = (x_1,\cdots, x_m)\}
%         \end{align*}
%         In terms of probabilities:
%         \begin{align*}
%             \Pbb(T>n+m) = \Pbb(T>n)\Pbb((X_{n+1},\cdots,X_{n+m}) = (x_1,\cdots, x_m)) = \Pbb(T>n)\prod\limits_{i=1}^m p_i
%         \end{align*}

%         Note that by the definition of expected value:
%         \begin{align*}
%             1 = \sum\limits_{n=0}^{\infty}\Pbb(T>n+m) = \prod\limits_{i=1}^m p_i\sum\limits_{n=0}^{\infty}\Pbb(T>n) = \prod\limits_{i=1}^mp_i \Ebb[T]
%         \end{align*}
%         Indeed, dividing through by $\prod_{i=1}^mp_i$ yields~\eqn{T_no_overlap}.

%         \item \textit{\textbf{Case 2: there is a pattern overlap of size $k$, which does not have an overlap itself.}} 
%         Suppose the pattern $(x_1,\cdots,x_m)$ has an overlapping subsequence $(x_1,\cdots,x_k)$ which itself does not have an overlap. Note that if $(x_1,\cdots,x_k)$ has an overlap, then we can repeat Case 2 by induction.

%         Define $T_y$ to be the next time after the first occurrence of the augmented pattern $(x_1,\cdots,x_m,y)$ it takes to observe the augmented pattern again. Then it is easy to see that $T_y > T$, that is:
%         \begin{align}\label{eq:T_overlap_k_1}
%             T_y = T + \Delta T
%         \end{align}
%         where $\Delta T$ is the time after the next occurrence of the original pattern $(x_1,\cdots,x_m)$ it takes to observe the next occurrence of the augmented pattern. Note that the computation of $\Ebb[T_y]$ is a simple instance of Case 1, since the addition of $y$ to the original sequence removes the overlap. Hence:
%         \begin{align*}
%             \Ebb[T_y] = \frac{1}{p_y\prod\limits_{i=1}^m p_i}
%         \end{align*}

%         We can compute $\Ebb[\Delta T]$ by conditioning on the next value $X$, assuming the sequence $(x_1,\cdots,x_m)$ has already been observed.
%         \begin{align*}
%             \Ebb[\Delta T | X = z] = \begin{cases}
%                 1 + \Ebb[T_y | x_1,\cdots,x_{k+1}] &\text{ if } z = x_{k+1}\\
%                 1 + \Ebb[T_y | x_1] &\text{ if } z = x_1\\
%                 1 &\text{ if } z = y\\
%                 1 + \Ebb[T_y] &\text{ if } z \not\in\{ x_1,x_{k+1},y\}
%             \end{cases}
%         \end{align*}
%         from which we can construct equations and compute $\Ebb[T]$. Namely:
%         \begin{align*}
%             \Ebb[\Delta T] = 1 + p_{k+1}\Ebb[T_y | x_1,\cdots,x_{k+1}] + p_1\Ebb[T_y | x_1] + (1 - p_{k+1} - p_1 - p_y)\Ebb[T_y]
%         \end{align*}
%         where $p_y$ denotes the probability of observing $y$ in a trial. Note that we can directly write, by definition,
%         \begin{align*}
%             \Ebb[T_y] &= \Ebb[T(x_1,\cdots,x_{k+1})] + \Ebb[T_y | x_1,\cdots,x_{k+1}]\\
%             \Ebb[T_y] &= \Ebb[T(x_1)] + \Ebb[T_y | x_1]
%         \end{align*}
%         where $T(x_1,\cdots,x_j)$ represents the time it takes to observe the next occurrence of the pattern $(x_1,\cdots,x_j)$ after its first occurrence. Since neither of the sequences $(x_1,\cdots,x_{k+1})$ nor $(x_1)$ have overlaps, we can use the first case to compute:
%         \begin{align*}
%             \Ebb[T(x_1,\cdots,x_{k+1})] = \frac{1}{\prod\limits_{i=1}^{k+1} p_i} , \ \ \Ebb[T(x_1)] = \frac{1}{p_1}
%         \end{align*}

%         In combination with~\eqn{T_overlap_k_1}, we get:
%         \begin{align*}
%             &\Ebb[T_y] = \Ebb[T] + 1 + p_{k+1}\left(\Ebb[T_y] - \Ebb[T(x_1,\cdots,x_{k+1})]\right) + p_1\left(\Ebb[T_y] - \Ebb[T(x_1)]\right)\\
%             &\hskip10.7cm + (1 - p_{k+1} - p_1 - p_y)\Ebb[T_y]\\
%             % \Longrightarrow \ &p_y\Ebb[T_y] = \Ebb[T] + \cancel{1} - p_{k+1}\Ebb[T(x_1,\cdots,x_{k+1})] - \cancel{p_1\Ebb[T(x_1)]}\\
%             \Longrightarrow \ &\Ebb[T] = \cancel{p_y}\cdot\frac{1}{\cancel{p_y}\prod\limits_{i=1}^m p_i} + p_{k+1}\cdot\frac{1}{\prod\limits_{i=1}^{k+1} p_i}
%         \end{align*}

%         In conclusion, where a specific pattern $(x_1,\cdots,x_m)$ has an overlap of size $k$
%         \begin{align*}
%             \Ebb[T] = \frac{1}{\prod\limits_{i=1}^m p_i} + \frac{1}{\prod\limits_{i=1}^{k} p_i}
%         \end{align*}    
%     \end{itemize}
% \end{proof}

% \violet{ FIX NOTATION:\\
% Suppose we are interested in computing the expected number of tosses $T$ of a coin with heads probability $p$ it takes to obtain a succession of $k$ heads in a row. While we can easily use the above formula for Case 1, one simple alternative method is to condition the umber of tosses on the outcome of the first toss.

% Use the regular definition of expectation:
% \begin{align*}
%     \Ebb[T] = \sum\limits_{i = 1}^k i\Pbb(T = i)
% \end{align*}
% Condition on the time of the first tail and rewrite the above equation:
% \begin{align*}
%     \Ebb[T] = \sum\limits_{i = 1}^k (1 - p)p^{i - 1}(i + \Ebb[T]) + kp^k
% \end{align*}
% Solve for $\Ebb[T]$:
% \begin{align*}
%     \Ebb[T] &= (1 - p)\sum\limits_{i = 1}^k ip^{i - 1} + \Ebb[T](1 - p)\sum\limits_{i = 1}^k p^{i - 1} + kp^k\\
%     &= (1 - p)\sum\limits_{i = 1}^k ip^{i - 1} + \Ebb[T](1 - p)\frac{1 - p^k}{1 - p} + kp^k\\
%     p^k\Ebb[T] &= (1 - p)\sum\limits_{i = 1}^k ip^{i - 1} + kp^k\\
%     \Ebb[T] &= \frac{1 - p}{p^k}\sum\limits_{i = 1}^k ip^{i - 1} + k = \frac{1}{p^k}\sum\limits_{i = 0}^{k - 1} p^i = \frac{(1 - p^k)}{p^k(1 - p)}
% \end{align*}
% }

% \begin{example}[String of Same Values]\label{ex:same_string}
%     Suppose we are interested in computing $T$ for a sequence of $m$ consecutive values, e.g. $(5,5,\cdots,5)$, for when $\Xcal := \{ 0,1,\cdots, 9\}$. Then following the analysis of Case 2 above, we can define $T_y$ for the augmented sequence $(5,5,\cdots, 5,y)$, where $y \neq 5$. Then we can compute $\Ebb[T]$ as follows:
%     \begin{align*}
%         \Ebb[T] = \Ebb[T_y] - \Ebb[\Delta T]
%     \end{align*}
%     where
%     \begin{align*}
%         \Ebb[T_y] = \frac{1}{p_5^mp_y}, \ \ \Ebb[\Delta T | X = z] = \begin{cases}
%             1 + \Ebb[\Delta T] &\text{ if } z = 5\\
%             1 + \Ebb[T_y] &\text{ if } z \not\in\{5,y\}\\
%             1 &\text{ if } z = y
%         \end{cases}
%     \end{align*}
%     so
%     \begin{align*}
%         &\Ebb[\Delta T] = 1 + p_5\Ebb[\Delta T] + (1 - p_5 - p_y)\Ebb[T_y]\\
%         \Longrightarrow &\Ebb[\Delta T] = \frac{1}{1 - p_5} + \frac{1 - p_5 - p_y}{1 - p_5}\cdot\Ebb[T_y]\\
%         \Longrightarrow &\Ebb[T] = \Ebb[T_y] - \Ebb[\Delta T] = -\frac{1}{1 - p_5} + \frac{p_y}{1 - p_5}\cdot\Ebb[T_y] = \frac{\frac{1}{p_5^{m}} - 1}{1 - p_5}
%     \end{align*}
%     which, one can verify, is the formula obtained when substituting it into Case 2.
% \end{example}

% \begin{example}[String of Same Values: Coin Tosses]\label{ex:same_string_coin}
%     Now we will consider a specific instance of~\exa{same_string} for when $\Xcal = \{ H, T\}$ and $p := \Pbb(X_n = H), q := 1-p = \Pbb(X_n = T)$. It is well-known that the formula of the time until one observes $m$ consecutive $H$'s is given by
%     \begin{align*}
%         \Ebb[T] = \sum\limits_{k=1}^{m}\frac{1}{p^k}
%     \end{align*}

%     We will derive this formula using the procedure used to prove Case 2 above. First, denote $T_T$ to be the time until we observe the sequence $(H,\cdots, H, T)$. Then
%     $\Ebb[T_y] = 1/(p^mq)$
%     \begin{align*}
%         \Ebb[\Delta T] = 1 + p\Ebb[\Delta T] + q\cdot 0 \ \Longrightarrow \ \Ebb[\Delta T] = \frac{1}{q}
%     \end{align*}
%     and
%     \begin{align*}
%         \Ebb[T] = \frac{1}{p^mq} - \frac{1}{q} = \frac{1 - p^m}{q} = \frac{(1-p)(1 + p + \cdots + p^{m-1})}{1 - p} = \sum\limits_{k=1}^{m}\frac{1}{p^k}
%     \end{align*}
%     which indeed verifies the formula.
% \end{example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% 5/20/2021 SOLVED PROBLEMS

% \begin{definition}[$k$-Record Values]
%     Let $X_1, X_2,\cdots$ be an iid sequence of random variables with $X_i \in \Zbb^{+}$. Then $X_n$ is a \textbf{$k$-record value} if $X_i \geq X_n$ for exactly $k$ of the values among $i = 1,\cdots,n$, including $n$.
% \end{definition}

% \begin{theorem}[Ignatov's Theorem]
%     % Let $V_k$ denote the ordered set of $k$-record values. Then $V_k, k \geq 1$ are iid random vectors. Furthermore, w
%     Let $X_1, X_2,\cdots$ be an iid sequence of random variables distributed according to the discrete, finite distribution over the compact range $\{1, \cdots, M\}$ where $M > 0$:
%     \begin{align*}
%         p_x := \begin{cases} \Pbb(X = x) &\text{ for } x = 1,\cdots, M\\
%         0 &\text{ for } x > M
%         \end{cases}
%     \end{align*}
%     define $T$ to be the ``$k$-record time'', i.e. the minimum time $T = n$ such that $X_n$ is a $k$-record value. Then
%     \begin{align*}
%         \Ebb[T] = (k-1)\sum\limits_{j=1}^{M-1}\lambda_j + k
%     \end{align*}
%     where
%     \begin{align*}
%         \lambda_x := \frac{p_x}{p_x + p_{x+1} + \cdots + p_M}
%     \end{align*}
%     is the renormalized probability of $x$.
% \end{theorem}

% \begin{proof}
%     Consider a specific sequence, and the corresponding subsequences $\{X^{(i)}\}$ constructed from isolating values which are $\geq i$ for $i\in\Zbb$.
%     % \begin{center}
%     %     \begin{tabular}{ l | c | c | c | c | c | c | c | c | c | c | c | c | c }
%     %     $\{X^{(1)}\}:$ & 2 & 5 & 1 & 6 & 9 & 8 & 3 & 4 & 1 & 5 & 7 & 8 & 2\\
%     %     $\{X^{(2)}\}:$ & 2 & 5 &  & 6 & 9 & 8 & 3 & 4 &  & 5 & 7 & 8 & 2\\ 
%     %     $\{X^{(3)}\}:$ &  & 5 &  & 6 & 9 & 8 & 3 & 4 &  & 5 & 7 & 8 & \\ 
%     %     $\{X^{(4)}\}:$ &  & 5 &  & 6 & 9 & 8 &  & 4 &  & 5 & 7 & 8 & \\ 
%     %     $\{X^{(5)}\}:$ &  & 5 &  & 6 & 9 & 8 &  &  &  & \circled{5} & 7 & 8 &
%     %     \end{tabular}
%     % \end{center}
%     Let $X_j^{(i)}$ be the $j$th element of subsequence $i$. Then $i$ is a $k$-record value iff $X_j^{(i)} = i$. This implies that the events $\{X_k^{(i)} = i\}$ are independent of each other over all $i$, 
%     % and
%     % \begin{align*}
%     %     \Pbb(j \in \{X^{(2)}\}) &= \Pbb(X = j | X \geq 2)\\
%     %     \Pbb(j \in \{X^{(3)}\}) &= \Pbb(X = j | X \geq 3)\\
%     %     &\vdots
%     % \end{align*}
%     and because the events $\{X_k^{(x)} = x\}$ are independent over all $x$ and independent of $k$, $V_k$ has the same distribution for all $k\geq 1$ and are independent of each other as well. Additionally, $\Pbb(X_j^{(x)} = x) = \Pbb(X = x | X \geq x)$, and we use this fact to compute $\Ebb[T]$. 

%     Denote
%     \begin{align*}
%         T_x := \min\{ n | X_j \geq X_n \text{ for exactly } k \text{ values of }(x,x+1,\cdots,M)\}
%     \end{align*}
%     That is, $T_i$ is the $k$-record value when all values of $X_j$ are known to be $\geq x$. We can compute its expected value by conditioning on the value of $X_k$:
%     \begin{align}\label{eq:k_record_value_i}
%         \Ebb[T_x] = \Ebb[T_x | X_k = x]\lambda_x + \Ebb[T_x | X_k > x](1 - \lambda_x)
%     \end{align}
%     Note that $\Ebb[T_x | X_k = x] = k$ since we are under the assumption that all values are $\geq x$. When $X_k > x$, the $k$-record value is no longer $x$. 
%     % Hence, we can renormalize the probabilities again with
%     % \begin{align*}
%     %     \alpha_i := \frac{p_j}{p_{i+1} + \cdots + p_m}, \ \text{ for } j = i+1,\cdots, m
%     % \end{align*}
%     % Then
%     % \begin{align*}
%     %     \Ebb[T_i | X_k > i] = \Ebb[T_{i+1} + N_i | X_k > i]
%     % \end{align*}
%     % where $N_i$ is the number of variables with value $i$ that need to be observed in order to obtain a $k$-record, and $T_{i+1}$ can be interpreted as the number of variables with value greater than $i$ that need to be observed for a $k$-record.

%     Note that the time to observe $r$ values larger than $x$, given that trial $k$ is greater than $i$ already, is equivalent to the number of trials it takes to obtain $r - 1$ successes, excluding the $k$th trial. Here, a success is interpreted as an outcome which yields value $> x$ given all outcomes are $\geq i$, and it occurs with probability $1 - \lambda_x$. Thus:
%     \begin{align*}
%         \Ebb[T_x | T_{x+1} = r, X_k > x] = 1 + \frac{r-1}{1 - \lambda_x} = \frac{r - \lambda_x}{1 - \lambda_x}
%     \end{align*}
%     where the $1 +$ comes from the inclusion of the $k$th trial, and the second equality comes from the fact that the expected time in between consecutive successes is $1/(1 - \lambda_x)$, like a Geometric random variable. Therefore, substituting this result in:
%     \begin{align*}
%         \Ebb[T_x | X_k > x] = \Ebb\left[ \frac{T_{x+1} - \lambda_x}{1 - \lambda_x} \bigg| X_k > x\right] = \frac{\Ebb[T_{x+1} | X_k > x] - \lambda_x}{1 - \lambda_x} = \frac{\Ebb[T_{x+1}] - \lambda_x}{1 - \lambda_x}
%     \end{align*}
%     where the conditioning disappears since $T_{x+1}$ already only counts trials which are $\geq x+1$.

%     Substituting the two components back into~\eqn{k_record_value_i} yields:
%     \begin{align*}
%         \Ebb[T_x] &= \Ebb[T_x | X_k = x]\lambda_x + \Ebb[T_x | X_k > x](1 - \lambda_x) = (k-1)\lambda_x + \Ebb[T_{x+1}]
%     \end{align*}

%     Then using induction on $x$ starting from $\Ebb[T_M] = k$ yields the general formula
%     \begin{align*}
%         \Ebb[T_x] = (k-1)\sum\limits_{j=x}^{M-1}\lambda_j + k
%     \end{align*}
%     and the result follows from the fact that $\Ebb[T] = \Ebb[T_1]$.
% \end{proof}

% \begin{example}[Second Largest vs Second Smallest]
%     \blue{EXAMPLE 3.27, P.127 ROSS, ItPM}\\
%     Consider the sequence of continuous iid random variables $X_1, X_2, \cdots \sim F$ with pdf $f = F'$.

%     Let $X_{(i),n}$ denote the $i$th-smallest value in the sequence observed up until time $n$, $X_1, \cdots, X_n$. Further denote
%     \begin{align*}
%         N := \min\{n\geq 2 | X_n = X_{(n-1),n}\}, \ \ \ M := \min\{n\geq 2 | X_n = X_{(2),n}\}
%     \end{align*}
%     That is, $N$ is the first time where $X_n$ is the second-largest value in the sequence $(X_1,\cdots,X_n)$ and $M$ is the first time where $X_n$ is the second-smallest. We are interested in determining which value, $X_N$ or $X_M$ tends to be the larger.

%     Define $E_n$ to be the event that $X_n$ is \textbf{not} the second-largest of $(X_1, \cdots, X_n)$. Then
%     \begin{align*}
%         \Pbb(N = n) = \Pbb(E_2\cap E_3\cap \cdots \cap E_{n-1}\cap \overline{E}_n)
%     \end{align*}

%     Since the $X_i$ are iid, knowing the rank ordering of $X_1, \cdots, X_n$ yields no information about their actual values. That means that the events $E_i$ are independent of each other over all $i$, and $X_i$ is equally likely to be the largest, or the second-largest, or $\cdots$, or the smallest. Thus,
%     \begin{align*}
%         \Pbb(E_i) = \frac{i-1}{i} \ \Longrightarrow \Pbb(N = n) = \frac{1}{2}\cdot\frac{2}{3}\cdot \cdots \frac{n-2}{n-1}\cdot\frac{1}{n} = \frac{1}{n(n-1)}
%     \end{align*}

%     We can then condition the value of $X_N$ on $N = n$:
%     \begin{align}\label{eq:second_largest_smallest_ex_1}
%         \Pbb(X_N = x) = \sum\limits_{n=2}^{\infty} \Pbb(X_N = x | N = n)\Pbb(N = n) = \sum\limits_{n=2}^{\infty} \frac{1}{n(n-1)}\cdot\Pbb(X_n = x)
%     \end{align}

%     Note that
%     \begin{align*}
%         \Pbb(X_{(i),n} \leq x) = \sum\limits_{k=i}^n \binom{n}{k} F(x)^k (1 - F(x))^{n-k}
%     \end{align*}
%     since by definition of $X_{(i),n}$, $X_{(i),n}$ will be less than or equal to $x$ iff at least $i$ of the $n$ values are $\leq x$. By taking derivatives:
%     \begin{align*}
%         \Pbb(X_{(i),n} = x) &= f(x)\sum\limits_{k=i}^n \binom{n}{k} kF(x)^{k-1} (1 - F(x))^{n-k} - f(x)\sum\limits_{k=i}^n \binom{n}{k} F(x)^{k} (n-k)(1 - F(x))^{n-k-1}\\
%         &= f(x)\left[ \sum\limits_{k=i}^n \frac{n!}{(n-k)!(k-1)!} F(x)^{k-1} (1 - F(x))^{n-k} - \sum\limits_{k=i}^n \frac{n!}{(n-k-1)!k!} F(x)^{k} (1 - F(x))^{n-k-1}\right]\\
%         &= f(x)\left[ \sum\limits_{k=i}^n \frac{n!}{(n-k)!(k-1)!} F(x)^{k-1} (1 - F(x))^{n-k} - \sum\limits_{j=i+1}^n \frac{n!}{(n-j)!(j-1)!} F(x)^{k} (1 - F(x))^{n-j}\right]\\
%         &= f(x)\cdot\frac{n!}{(n-i)!(i-1)!}\cdot F(x)^{i-1}(1 - F(x))^{n-i}
%     \end{align*}

%     With $i = n-1$ and substituting the above expression into~\eqn{second_largest_smallest_ex_1} yields
%     \begin{align*}
%         \Pbb(X_N = x) &= \sum\limits_{n=2}^{\infty} \frac{1}{n(n-1)}\cdot\frac{n!}{(n-2)!} f(x)F(x)^{n-2}(1 - F(x))\\
%         &= f(x)(1 - F(x))\sum\limits_{n=2}^{\infty} F(x)^{n-2}\\
%         &= f(x)(1 - F(x))\cdot \frac{1}{1 - F(x)} \ \text{ by geometric series}\\
%         &= f(x)
%     \end{align*}

%     This implies that $X_N \sim X_1$. To obtain the distribution of $X_M$, just invert the sign and repeat the previous calculation since the second-smallest of $X_1, \cdots, X_n$ and be interpreted as the second-largest of $-X_1, \cdots, -X_n$. Thus, $-X_M \sim -X_1$ and so $X_M \sim X_1$. 

%     Therefore, whether $X_M \leq X_N$ or $X_M > X_N$ is determined completely randomly according to the distribution $F$. One might note the analogy to the well-known basic probability of computing $\Pbb(U_1 \leq U_2)$ for two iid random variables $U_1$ and $U_2$.
% \end{example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% 5/7/2021 LECTURE

% \red{EXAMPLES 7.9.2, 7.9.3\\
% FIX NOTATION:\\
% \textbf{Mean Time to a Maximal Run of Different Values}\\

% Suppose $X_i, i \geq 1$ are iid random variables that are equally likely to take on any of the values $1,2, \cdots m$. After being observed sequentially, let $T$ be the first time that a run of $m$ consecutive values includes all the values $1, 2, \cdots m$.
% \begin{align*}
%     T = \min\{ n: X_{n - m + 1}, \cdots, X_n \text{ are all distinct}\}
% \end{align*}

% We desire to compute $\Ebb[T]$. Define a renewal process where the first renewal occurs at time $T$, from which you restart and, let the next renewal occur the next time a run of $m$ consecutive values are all different.

% Now transform the renewal process into a delayed renewal reward process by assuming that a reward of 1 is earned at time $n$, for $n \geq m$, if the values $X_{n - m + 1}, \cdots, X_n$ are all distinct, i.e, a reward is earned each time the previous $m$ values are all distinct.

% % Let $R_i$ denote the reward earned at time $i$. Then by property of renewal reward processes, we have:
% % \begin{align*}
% %     \lim_{n} \frac{E\left(\sum\limits_{i = 1}^n R_i\right)}{n} = \frac{\Ebb[R]}{\Ebb[T]}
% % \end{align*}
% % where $R$ is the rewards earned between renewal periods.

% With $A_i$ equal to the set of the first $i$ data values of a renewal run, and $B_i$ to the set of the first $i$ values after this renewal run, we get that:
% \begin{align*}
%     \Ebb[R] &= 1 + \sum\limits_{i = 1}^{m - 1}\Ebb[\text{reward earned at time $i$ after a renewal})\\
%     &= 1 + \sum\limits_{i = 1}^{m - 1}\Pbb(A_i = B_i)\\
%     &= 1 + \sum\limits_{i = 1}^{m - 1} \frac{i!}{m^i}\\
%     &= \sum\limits_{i = 0}^{m - 1} \frac{i!}{m^i}
% \end{align*}

% Furthermore, for $i \geq m$, we have that
% \begin{align*}
%     \Ebb[R_i] &= \Pbb(X_{i - m + 1}, \cdots, X_i \text{ are all different}) = \frac{m!}{m^m}
% \end{align*}

% Then it follows from the property of renewal reward processes that
% \begin{align*}
%     \frac{m!}{m^m} &= \frac{\Ebb[R]}{\Ebb[T]}
% \end{align*}
% and we finally obtain that
% \begin{align*}
%     \Ebb[T] &= \frac{m^m}{m!}{\Ebb[R]} = \frac{m^m}{m!}\sum\limits_{i = 0}^{m - 1} \frac{i!}{m^i}
% \end{align*}

% Now consider the following example: continually flip a coin that lands heads with probability $p$ and tails with probability $q = 1 - p$. We shall compute the expected time until the pattern $HHHTHHH$ occurs.

% Construct a renewal process by letting the first renewal occur when the pattern first appears, and then start over. Say that a reward of 1 is earned whenever the pattern appears.

% If $R$ denotes the reward earned between renewal periods, we have
% \begin{align*}
%     \Ebb[R] &= 1 + \sum\limits_{i = 1}^6 \Ebb[\text{reward earned at time $i$ after a renewal})\\
%     &= 1 + 0 + 0 + 0 + p^3q + p^3qp + p^3qp^2
% \end{align*}
% where each sum term after 1 arises from the patterns $H$, $HH$, $HHH$, $HHHT$, $HHHTH$, and $HHHTHH$ respectively.

% We have that the expected reward earned at time $i$ is $\Ebb[R_i] = p^6q$ (because the pattern we desire to observe has six heads and one tails)\\

% From the renewal reward property:
% \begin{align*}
%     \frac{1 + qp^3 + qp^4 + qp^5}{\Ebb[T]} &= qp^6\\
%     \Ebb[T] &= \frac{1}{qp^6} + \frac{1}{p^3} + \frac{1}{p^2} + \frac{1}{p}
% \end{align*}

% \textbf{Increasing Runs of Continuous Random Variables}\\

% Say we have a sequence of iid random variables $X_1, X_2, \cdots$.  Let $T$ denote the first time there is a string of $r$ consecutive increasing values:
% \begin{align*}
%     T = \text{min}\{ n \geq r : X_{n - r + 1} < X_{n - r + 2} < \cdots < X_n\}
% \end{align*}

% To compute $\Ebb[N(n)]$, define a stochastic process whose state at time $k$, called $S_k$, is equal to the number of consecutive increasing values starting from time $k$. That is, for $1 \leq j \leq k$,
% \begin{align*}
%     S_k = j \text{ if } X_{k - j} > X_{k - j + 1} < \cdots < X_{k - 1} < X_k
% \end{align*}

% Note that a renewal occurs at time $k$ iff $S_k = ir$ for some $i \geq 1$. For instance, if $r = 3$ and $X_5 > X_6 > \cdots > X_{11}$, then we have $S_6 = 1, S_7 = 2, \cdots , S_{11} = 6$. Hence:
% \begin{align*}
%     \Pbb(S_k = j) &= \Pbb(X_{k - j} > X_{k - j + 1} < \cdots < X_{k - 1} < X_k)\\
%     &= \Pbb(X_{k - j + 1} < \cdots < X_{k - 1} < X_k) - \Pbb(X_{k - j} < X_{k - j + 1} < \cdots < X_{k - 1} < X_k)\\
%     &= \frac{1}{j!} - \frac{1}{(j + 1)!}\\
%     &= \frac{j}{(j + 1)!}
% \end{align*}
% since all possible orderings of random variables are equally likely.

% So we see that
% \begin{align*}
%     &\lim_{k \rightarrow \infty} \Pbb(\text{a renewal occurs at time } k)\\
%     &= \lim_{k \rightarrow \infty} \sum\limits_{i = 1}^\infty \Pbb(S_k = ir)\\
%     &= \sum\limits_{i = 1}^\infty \frac{ir}{(ir + 1)!}
% \end{align*}

% Using the tail sum formula for expectations, we conclude that
% \begin{align*}
%     \Ebb[N(n)] = \sum\limits_{k = 1}^n \Pbb(\text{a renewal occurs at time } k)
% \end{align*}

% So we finally obtain that
% \begin{align*}
%     \Ebb[T] = \left(\sum\limits_{i = 1}^\infty \frac{ir}{(ir + 1)!}\right)^{-1}
% \end{align*}
% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% rather than a sequence composed entirely of heads or tails, e.g. $A := HHTTHH$ and $B := HTHTT$.
% % \begin{example}[Coin Tosses: Specific Strings]\label{ex:min_strings}
% % \blue{(PROBLEM 3.22)}\\
% Suppose
%  % we are given a coin with probability of heads $p$, and 
% we are interested in comparing the two specific sequence patterns. 
% Let $T(A)$ and $T(B)$ denote the number of flips until we observe $A$ and $B$, respectively. 
%METHODOLOGY FROM EXAMPLE 3.5(A).
% We are interested in the probability that $A$ will occur before $B$ as well as the expected time it takes to observe either one of the patterns $A$ or $B$. We further denote $T(B|A)$ to be the additional number of flips needed in order to observe $B$ in the sequence, given we've already observed $A$. Likewise, define $T(A|B)$. Further denote $P_A$ to be the probability that $A$ will occur before $B$. Further denote $T_{\text{min}} := \min\{T(A),T(B)\}$. We can derive a system of equations with these variables as follows:
% \begin{align*}
%     \Ebb[T(A)] &= \Ebb[T_{\text{min}}] + \Ebb[T(A)-T_{\text{min}}] = \Ebb[T_{\text{min}}] + \Ebb[T(A|B)](1-P_A) + 0\cdot P_A\\
%     \Ebb[T(B)] &= \Ebb[T_{\text{min}}] + \Ebb[T(B)-T_{\text{min}}] = \Ebb[T_{\text{min}}] + \Ebb[T(B|A)]P_A + 0\cdot(1-P_A)
% \end{align*}
% Solving for the variables yields
% \begin{align*}
%     P_A &= \frac{\Ebb[T(B)] + \Ebb[T(A|B)] - \Ebb[T(A)]}{\Ebb[T(B|A)] + \Ebb[T(A|B)]},\qquad \Ebb[T_{\text{min}}] = \Ebb[T(B)] - \Ebb[T(B|A)]P_A
% \end{align*}

% For example, in the specific case of $A := HHTTHH$ and $B := HTHTT$, we get from~\thm{pattern_occurrence_discrete}:
% \begin{align*}
%     \Ebb[T(A)] = \frac{1}{p^4q^2} + \frac{1}{p^2} + \frac{1}{p}, \ \ \Ebb[T(B)] = \frac{1}{p^2q^3}
% \end{align*}
% and
% \begin{align*}
%     \Ebb[T(B|A)] &= \Ebb[T(B)] - \Ebb[T(H)] = \frac{1}{p^2q^3} - \frac{1}{p}\\
%     \Ebb[T(A|B)] &= \Ebb[T(A)] = \frac{1}{p^4q^2} + \frac{1}{p^2} + \frac{1}{p}
% \end{align*}
% where the first equation follows since the $H$ at the end of sequence $A$ can be reused, while the second equation follows because there is no subsequence at the end of sequence $B$ which can be reused for $A$. 
% For $p=\frac{1}{3}$, the formula yields
% \begin{align*}
%     P_A = \frac{p^2}{p^2q^3 + q + p^2} = \frac{27}{197}, \qquad \Ebb[T_{\text{min}}] = \frac{1}{p^2q^3} - \left( \frac{1}{p^2q^3} - \frac{1}{p}\right)P_A = \frac{20979}{788}
% \end{align*}

% Now, consider Bernoulli trials with $H$ probability $p$ and $T$ probability $q := 1-p$. We can use the above generic formula to compute the probability $P_A$ that a sequence of $m$ heads, denoted by sequence $A$, is observed before a sequence of $n$ tails, denoted by sequence $B$. We first have
% \begin{align*}
%     T_A = \sum\limits_{i=1}^m \frac{1}{p^i}, \ \ T_B = \sum\limits_{j=1}^n \frac{1}{q^j}
% \end{align*}
% Note that since neither of the sequences overlap with each other, $T_{A|B} = T_A$ and $T_{B|A} = T_B$. Hence:
% \begin{align*}
%     T_A &= T_{\text{min}} + (T_A - T_{\text{min}}) = T_{\text{min}} + (1 - P_A)T_{A|B}\\
%     T_B &= T_{\text{min}} + (T_B - T_{\text{min}}) = T_{\text{min}} + P_AT_{B|A}
% \end{align*}
% and thus,
% \begin{align*}
%     P_A 
%     % &= \frac{\sum\limits_{j=1}^n \frac{1}{q^j}}{\sum\limits_{i=1}^m \frac{1}{p^i} + \sum\limits_{j=1}^n \frac{1}{q^j}} = \frac{\frac{1 - \frac{1}{q^n}}{q\left(1 - \frac{1}{q}\right)}}{\frac{1 - \frac{1}{p^m}}{p\left(1 - \frac{1}{p}\right)} + \frac{1 - \frac{1}{q^n}}{q\left(1 - \frac{1}{q}\right)}} 
%     = \frac{(1 - q^n)p^{m-1}}{q^{n-1} + p^{m-1} - p^{m-1}q^{n-1}}
% \end{align*}
% \end{example}

% \red{
% \begin{example}[Computing for $m$ Successes Using Generating Functions]
%     \blue{FELLER SECTION 7 AND 8. TODO: INCLUDE THE "before $n$ failures" CONDITIONING.}\\
%     We can perform and alternative method of computation as in~\exa{min_strings} using generating functions. Let $E$ denote the event that $m$ successes occurs. Denote $u_n$ to be the probability that $E$ occurs at trial $n$ and denote $f_n$ to be the probability that $E$ \textit{first} occurs at trial $n$. We take as convention $f_0 := 0$ and $u_0 := 1$ and denote their corresponding generating functions as
%     \begin{align*}
%         F(s) = \sum\limits_{k=1}^{\infty} f_ks^k, \ \ U(s) = \sum\limits_{k=0}^{\infty} u_ks^k
%     \end{align*}

%     Note that the probability that $E$ occurs for the first time at trial $k$, then again at trial $n>k$ is $f_ku_{n-k}$. Hence, conditioning on $k$ yields the recursive relationship
%     \begin{align}\label{eq:generating_recursion}
%         u_n = f_1u_{n-1} + f_2u_{n-2} + \cdots + f_nu_0 =: \{f_i\} * \{u_i\}
%     \end{align}

%     Transforming~\eqn{generating_recursion} into generating functions yields
%     \begin{align}\label{eq:u_f_gen_fcns}
%         U(s) - 1 = F(s)U(s) \ \Longrightarrow \ U(s) = \frac{1}{1 - F(s)}
%     \end{align}

%     Recall that for Bernoulli random variables 
%     \begin{align}\label{eq:bernoulli_gen_fcn}
%         U(s) = \frac{1 - qs}{1 - s}, \ \ F(s) = \frac{ps}{1 - qs}
%     \end{align}

%     Furthermore, the probability of observing a string of $m$ successes is given by $p^m$. Using~\eqn{generating_recursion}, we get
%     \begin{align}\label{eq:generating_recursion_bernoulli}
%         p^m = u_n + u_{n-1}p + \cdots u_{n-m+1}p^{m-1}
%     \end{align}

%     Hence, we can rewrite the recursive equation in the following way by multiplying across the equation by $s^n$ and summing over all $n \geq m$:
%     \begin{align*}
%         \sum\limits_{n=m}^{\infty} p^ms^n = \sum\limits_{n=m}^{\infty} \left( u_ns^n + u_{n-1}ps^n + \cdots u_{n-m+1}p^{m-1}s^n \right)
%     \end{align*}

%     We simplify the entire equation by changing variables from $k = n-m$:
%     \begin{align*}
%         &\sum\limits_{k=0}^{\infty} p^ms^{m+k} = \sum\limits_{k=0}^{\infty}\left( u_{k+m}s^{k+m} + u_{k+m-1}ps^{k+m} + \cdots u_{k+1}p^{m-1}s^{k+m} \right)\\
%         \Longrightarrow & \ p^ms^m\sum\limits_{k=0}^{\infty} p^ms^k = (U(s) - 1)\sum\limits_{k=0}^{m-1} (ps)^k\\
%         \Longrightarrow & \ \frac{p^ms^m}{1-s} = (U(s) - 1)\cdot\frac{1 - (ps)^m}{1 - ps}
%     \end{align*}

%     From geometric series, the left side yields:
%     \begin{align*}
%         \sum\limits_{n=m}^{\infty} p^ms^n = p^ms^m\sum\limits_{k=0}^{\infty} p^ms^k = \frac{p^ms^m}{1-s}
%     \end{align*}
%     and the right side sum can be rearranged as follows
%     \begin{align*}
%         &\sum\limits_{k=0}^{\infty}\left( u_{k+m}s^{k+m} + u_{k+m-1}ps^{k+m} + \cdots u_{k+1}p^{m-1}s^{k+m} \right)\\
%         &\hskip1cm = \left( u_ms^m + u_{m+1}s^{m+1} + u_{m+2}s^{m+2} + \cdots \right)\left( 1 + ps + \cdots p^{m-1}s^{m-1}\right)\\
%         &\hskip1cm = (U(s) - 1)\sum\limits_{k=0}^{m-1}(ps)^k = (U(s) - 1)\cdot\frac{1 - (ps)^m}{1 - ps}
%     \end{align*}
%     % Using~\eqn{bernoulli_gen_fcn} and the Geometric series formula, the equation yields
%     % \begin{align*}
%     %     (U(s) - 1)(p^{m-1}s^{m-1} + p^{m-2}s^{m-2} + \cdots ps + 1) = \frac{p^ms^m}{1-s}
%     % \end{align*}

%     Therefore,
%     \begin{align*}
%         U(s) = \frac{1 - s + qp^ms^{m+1}}{(1-s)(1 - p^ms^m)}
%     \end{align*}

%     Using~\eqn{u_f_gen_fcns}, we get
%     \begin{align*}
%         F(s) = \frac{p^ms^m(1 - ps)}{1 - s + qp^ms^{m+1}}
%     \end{align*}
%     Note that $F(s)$ is the generating function of the recurrence times.

%     % Recall that the probability mass function is then recovered by taking derivatives:
%     % \begin{align*}
%     %     \Pbb(m \text{ successes by time }n) = \frac{1}{n!}U^{(n)}(0), \ \ \Pbb(\text{first }m \text{ successes by time }n) = \frac{1}{n!}F^{(n)}(0)
%     % \end{align*}

%     \begin{align*}
%         U'(s) = \frac{((m+1)qp^ms^m - 1)(1-s)(1-p^ms^m) - (1 - s + qp^ms^{m+1})[(p^ms^m - 1) - m(1-s)p^ms^{m-1}]}{(1 - s)^2(1 - p^ms^m)^2}
%     \end{align*}

%     To obtain the expression in the original time-domain area, take the limit as $s\to 1$. This requires the application of L'Hopital's Rule:
%     \begin{align*}
%         \lim_{s\to 1} U(s) &= \lim_{s\to 1}\frac{1 - s + qp^ms^{m+1}}{(1-s)(1 - p^ms^m)} = \lim_{s\to 1} \frac{-1 + qp^m(m+1)s^m}{-(1 - p^ms^m) - (1-s)p^mms^{m-1}} = \frac{(m+1)qp^m}{p^m-1}
%     \end{align*}

%     \blue{??}
% \end{example}
% }

% \begin{example}[Coin Tosses: First $k$]
%     \blue{(PROBLEM 3.23)}\\
%     Suppose that the first $k$ outcomes of flipping a coin with probability $p$ of yielding heads is observed, and $N$ is the additional number of flips after the first $k$ which are required in order to observe the same sequence of $k$ outcomes.

%     Consider the specific case where $k = 3$. There are $2^3 = 8$ total different possible sequences that can appear at the beginning of the sequence. The probabilities of occurrence for a coin with probability $p$ of yielding heads are listed below:
%     \begin{align*}
%         &p(H,H,H) = p^3, \ p(H,H,T) = p^2q\\
%         &p(H,T,H) = p^2q, \ p(T,H,H) = p^2q\\
%         &p(H,T,T) = pq^2, \ p(T,H,T) = pq^2\\
%         &p(T,H,T) = pq^2, \ p(T,T,T) = q^3
%     \end{align*}
%     The distribution of $N$ can then be determined as a geometric random variable by the \violet{strong law for delayed renewal processes.} For general $k$, we can write:
%     \begin{align*}
%         \Ebb[T] &= \sum\limits_{(x_1,\cdots,x_k) \in \{H,T\}^k}\Ebb[T|(x_1,\cdots,x_k)]p(x_1,\cdots,x_k)\\
%         &= \sum\limits_{(x_1,\cdots,x_k) \in \{H,T\}^k}\frac{1}{p(x_1,\cdots,x_k))}\cdot p(x_1,\cdots,x_k)\\
%         &= \sum\limits_{(x_1,\cdots,x_k) \in \{H,T\}^k} 1 = 2^k
%     \end{align*}
%     where the penultimate equality comes from the geometric distribution.
% \end{example}

\begin{remark}[Alternative Pattern-Occurrence Problem with Random Walks]
    If we are interested in keeping track of longer pattern sequences of impulsive disturbances, the pattern-occurrence problem can also be solved using an alternative approach with random walks. Borrowing influence from common motivational problems such as the Gambler's Ruin problem, the theory of random walks can be used to determine the expected time it takes the system to reach certain boundaries imposed on the system state, upon which the modulation control mechanism takes over. For the sake of keeping this paper focused, we defer discussion of the connections between the pattern-occurrence problem and the theory of random walks to~\cite{han21book}. A comprehensive treatment of random walk theory background needed to understand these connections can also be found in~\cite{han21book}.
\end{remark}


==> arxiv_sections/pattern_occurrence_new_detailed.tex <==
%%%%% VERSION OF PATTERN OCCURRENCE SECTION WITH NEW NON-ROSS EXAMPLE. FOR THE BOATLOAD OF COMMENTED OUT MATERIAL, SEE pattern_occurrence.tex.

With the renewal theory background established, we now consider the general problem of \textit{pattern occurrence}. We first discuss a motivational example before describing a more general result. 

\begin{example}[Motivating Example: Expected Time]\label{ex:brute_force}
    Suppose that we are observing a sequence of iid binary random variables $X_1, X_2, \cdots$, each with distribution
    \begin{align*}
        X_i = \begin{cases}
            1 &\text{ with probability } \ p\\
            0 &\text{ with probability } \ q := 1-p
        \end{cases}
    \end{align*}
    Suppose we designate two strings $A_1$ and $A_2$ composed of $0$'s and $1$'s. One common problem of interest is the expected number of trials it takes to observe two consecutive instances of $A_1$ in the sequence $\{X_i\}_{i=1}^{\infty}$; likewise, for $A_2$.

    We choose for concreteness $A_1 := 1,0,1,0,\cdots,1,0$ to be the length-$2n$ alternating sequence of $1$ and $0$, and $A_2 := 1,\cdots,1,0,\cdots,0$ to be the length-$m$ string of all $1$'s followed by the length-$m$ string of all $0$'s. 

    Denote $T_i$ to be the time in between two consecutive instances of $A_i$, where $i=1,2$. We first compute $\Ebb[T_1]$. Note that if we were to treat each pair of $(1,0)$ as a single symbol, then we can view $A_1$ as a length-$n$ string composed entirely of $(1,0)$ pairs. Note that the probability of observing exactly $(1,0)$ is $pq$. Hence, the number of trials required to observe $(1,0)$ for the first time after the last occurrence of $A_1$ is distributed according to a Geometric random variable with parameter $pq$. Using an intuitive argument, we can now iteratively derive the expression for the expected time it takes to obtain a new string of $n$ pairs of $(1,0)$ after the last occurrence. 

    Note that if $(1,0)$ appears on the spot, we are done, because we can combine this new $(1,0)$ with the last $n-1$ occurrences of $(1,0)$ from the last instance of $A_1$ to create the new instance of $A_1$. However, if $(1,0)$ doesn't appear exactly, we need to restart as if we were observing $A_1$ from scratch. The expected time it takes to observe the first instance of $(1,0)$ is $1/(pq)$ due to the Geometric distribution. Once the first $(1,0)$ has been observed, the time it takes to observe the second instance of $(1,0)$ is also Geometrically distributed, but with parameter $p^2q^2$ because we must observe the two $(1,0)$'s consecutively; the probability of observing exactly the sequence $(1,0,1,0)$ is thus $p^2q^2$. Hence, we have that the mean number of trials to observe two consecutive $(1,0)$'s for the first time is $(1/(pq)) + (1/(pq)^2)$. 

    Iterating this argument until $n$ consecutive $(1,0)$'s, we have that the expected number of trials to in between consecutive instances of $A_1$ is:
    \begin{align}\label{eq:motive_success_time}
        \Ebb[T_1] = \sum\limits_{j=1}^n \frac{1}{(pq)^j}
    \end{align}

    The expression~\eqn{motive_success_time} can also be directly derived using a system of linear equations. Denote $E_{n,j}$ to be the expected number of trials needed to observe $n$ consecutive $(1,0)$'s given $j$ consecutive $(1,0)$'s, where $0\leq j\leq n$, have already been observed. Further denote $E_{n,j}^{(1)}$ to be the expected number of trials needed to observe $n$ consecutive $(1,0)$'s given $j$ consecutive $(1,0)$'s and an additional trial with outcome $1$ has been observed. We now have $n$ equations with these variables set up as follows:
    \begin{align*}
        E_{n,n-k} &= 1 + pE_{n,n-k}^{(1)} + qE_{n,0}\\
        E_{n,n-k}^{(1)} &= 1 + pE_{n,0}^{(1)} + qE_{n,n-k+1}, \ \ \forall 2\leq k\leq n\\
        E_{n,n} &= 1
    \end{align*}

    Note that we can simplify the two equations and remove the intermediate variables $E_{n,n-k}^{(1)}$, for $1\leq k\leq n-1$ via substitution:
    \begin{align*}
        E_{n,n-k} = 1 + p + p^2E_{n,0}^{(1)} + pqE_{n,n-k+1} + qE_{n,0}
    \end{align*}

    We can then solve for the remaining variables by iterating from $k=n$ to $k=2$:
    \begin{align*}
        E_{n,0}^{(1)} &= E_{n,1} + \frac{1}{q}\\
        E_{n,0} &= E_{n,1} + \frac{1}{q} + \frac{1}{p} = E_{n,1} + \frac{1}{pq}\\
        E_{n,1} &= E_{n,2} + \frac{1}{(pq)^2}\\
        &\vdots\\
        E_{n,k} &= E_{n,k+1} + \frac{1}{(pq)^k}
    \end{align*}
    and setting $\Ebb[T_1] = E_{n,0}$ yields the same expression as in~\eqn{motive_success_time}.

    We compute $\Ebb[T_2]$ using a similar approach. Unlike the pattern $A_1$, there is no subsequence from the end of the last instance of $A_2$ which we can reuse as a part of the next instance of $A_2$. We effectively need to count the number of trials as if we were starting the sequence from scratch. 

    We must first observe the $m$ consecutive $1$'s before considering the $m$ consecutive $0$'s. Note that the probability of observing exactly $m$ consecutive $1$'s is $p^m$; hence, the time it takes to observe $m$ consecutive $1$'s is Geometrically distributed with parameter $p^m$. Once $m$ $1$'s have been observed, the time it takes to observe $m$ consecutive $0$'s is also Geometrically distributed. However, with the same argument used for $A_1$, the $m$ consecutive $0$'s must follow immediately after the $m$ consecutive $1$'s. Thus, the time to observe $A_2$ is Geometrically distributed with parameter $p^mq^m$. Likewise:
    \begin{align}\label{eq:motive_failure_time}
        \Ebb[T_2] = \frac{1}{(pq)^m}
    \end{align}

    The expression~\eqn{motive_failure_time} can also be derived by solving a system of equations. Denote $E_{k,i}$ for $0\leq k\leq m$ and $i=0,1$ to be the expected number of trials needed to observe the full $A_2$ given we have observed the subsequence of $A_2$ up to the $k$th outcome of $i$. Then the equations are
    \begin{align*}
        E_{k,1} &= 1 + pE_{k+1,1} + qE_{0,1}, \ \ \forall \ 0\leq k\leq m-1\\
        E_{m,1} &= 1 + pE_{m,1} + qE_{1,0},\\
        E_{k,0} &= 1 + pE_{1,1} + qE_{k+1,0}, \ \ \forall \ 1\leq k\leq m\\
        E_{m,0} &= 1
    \end{align*} 

    From the first $m$ equations, we get that:
    \begin{align*}
        E_{1,1} = E_{m,1} + \frac{1}{p^2} + \cdots + \frac{1}{p^m} = E_{m,1} + \underbrace{\frac{p(1 - p^{m-2})}{qp^m}}_{=: K}
    \end{align*}
    and from the next $m+1$ equations, we get:
    \begin{align*}
        E_{1,0} &= E_{m,1} - \frac{1}{q} = E_{1,1} - K - \frac{1}{q}\\
        E_{k,0} &= E_{1,1} - \frac{1}{q^{k-1}}\left( K + \frac{1}{q}\right) - \frac{1}{q^{k-1}} - \cdots - \frac{1}{q}, \ \ \forall \ 2\leq k\leq m
    \end{align*}

    In particular, substituting $k = m$ and using the boundary condition:
    \begin{align*}
        1 = E_{m,0} &= E_{1,1} - \frac{1}{q^{m-1}}\left( K + \frac{1}{q}\right) - \frac{1}{q^{m-1}} - \cdots - \frac{1}{q}\\
        \Longrightarrow E_{0,1} &= \frac{1}{p} + 1 + \frac{1}{q^{m-1}}\left( \frac{p(1 - p^{m-2})}{qp^m} + \frac{1}{q}\right) + \frac{q(1 - q^{m-1})}{pq^m}
    \end{align*}
    and simplification of the expression yields the expression~\eqn{motive_failure_time}.
\end{example}

\begin{example}[Motivating Example: Probability]\label{ex:brute_force_ctd}]
    Given a sequence of binary random variables $X_1, X_2, \cdots$, another problem of interest is the probability of observing one subsequence before another. We consider solving a generalization of a simple problem from~\cite{ross10book} \blue{chapter number and check which Ross book it is}. Let $A_1$ be a string of $n$ $1$'s, $A_2$ be a string of $m$ $0$'s, and $A_3$ be a string of $r$ $2$'s, where $n, m, r\in\Nbb^{+}$. Suppose the values of $\{X_i\}_{i=1}^{\infty}$ are generated in the following way. Until one of the two sequences $A_1$ or $A_2$ have been observed:
    \begin{align*}
        X_i = \begin{cases}
            1 &\text{ with probability } \ p_1\\
            0 &\text{ with probability } \ q_1 := 1-p_1
        \end{cases}
    \end{align*}
    If $A_1$ is observed first, the $X_i$ take the following distribution until either $A_2$ or $A_3$ is observed:
    \begin{align*}
        X_i = \begin{cases}
            2 &\text{ with probability } \ p_2\\
            0 &\text{ with probability } \ q_2 := 1-p_2
        \end{cases}
    \end{align*}
    Otherwise, if $A_2$ is observed first, the $X_i$ take the following distribution until either $A_1$ or $A_3$ is observed:
    \begin{align*}
        X_i = \begin{cases}
            1 &\text{ with probability } \ p_3\\
            2 &\text{ with probability } \ q_3 := 1-p_3
        \end{cases}
    \end{align*}

    Given this setup, we are interested in the probability $P_{1,3}$ that $A_1$ is observed before $A_2$, and then $A_3$ is observed before $A_2$. Denote $\Ecal_1$ to be the event that $A_1$ is observed before $A_2$, and let $P_1 := \Pbb(\Ecal_1)$. Further denote $\Ecal_3$ to be the event that $A_3$ is observed before $A_2$ given $A_1$ has been observed first, and let $P_3 := \Pbb(\Ecal_3)$. Then by conditional probability, we can decompose the probability into two parts:
    \begin{align*}
        P_{1,3} = P_1P_3
    \end{align*}

    Now $P_1$ and $P_3$ can then be computed independently. We first compute $P_1$ by conditioning on the outcome of the first trial $X_1$. To that end, we denote $\Scal_1$ to be the event that $X_2=\cdots=X_n=1$ and $\Scal_0$ to be the event that $X_2=\cdots=X_m = 0$. Thus:
    \begin{align}\label{eq:motive_prob_eq1}
        P_1 := \Pbb(\Ecal) &= p_1\Pbb(\Ecal|X_1=1) + q_1\Pbb(\Ecal|X_1=0)\notag\\
        &= p_1\left(p_1^{n-1}\Pbb(\Ecal|X_1=1,\Scal_1) + (1 - p_1^{n-1})\Pbb(\Ecal|X_1=1,\Scal_1^{c})\right)\notag\\
        &\hskip1cm + q_1\left( q_1^{m-1}\Pbb(\Ecal|X_1=0,\Scal_0) + (1 - q_1^{m-1})\Pbb(\Ecal|X_1=0,\Scal_0^{c})\right)
    \end{align}
    Note that $\Pbb(\Ecal|X_1=1,\Scal_1) = 1$ and $\Pbb(\Ecal|X_1=0,\Scal_0) = 0$. Furthermore, $\Pbb(\Ecal|X_1=0) = \Pbb(\Ecal|X_1=1,\Scal_1^{c})$ because $\Scal_1^{c}$ means that the outcome is $0$ for one of the trials among $X_2, \cdots, X_n$, after which we need to restart the count; the probability then becomes equivalent to $\Pbb(\Ecal|X_1=0)$. Likewise, $\Pbb(\Ecal|X_1=1) = \Pbb(\Ecal|X_1=0,\Scal_0^{c})$. Note then we now have a system of two equations:
    \begin{align*}
        \Pbb(\Ecal|X_1=1) = p_1^{n - 1} + (1 - p_1^{n - 1})\Pbb(\Ecal|X_1=0), \qquad \Pbb(\Ecal|X_1=0) = (1 - q_1^{m-1})\Pbb(\Ecal|X_1=1)
    \end{align*}
    which we can solve and substitute back into~\eqn{motive_prob_eq1}:
    \begin{align}\label{eq:motive_prob}
        P_1 = \eqn{motive_prob_eq1} &= p_1\left(p_1^{n-1} + (1 - p_1^{n-1})\Pbb(\Ecal|X_1=0)\right) + q_1(1 - q_1^{m-1})\Pbb(\Ecal|X_1=1)\notag\\
        &= \frac{q_1^{m - 1}(1 - p_1^n)}{p_1^{n - 1} + q_1^{m - 1} - p_1^{n - 1}q_1^{m - 1}}
    \end{align}

    Note that $P_3$ can be computed using the same formula~\eqn{motive_prob}:
    \begin{align*}
        P_3 = \frac{q_2^{m - 1}(1 - p_2^n)}{p_2^{n - 1} + q_2^{m - 1} - p_2^{n - 1}q_2^{m - 1}}
    \end{align*}

    Hence:
    \begin{align*}
        P_{1,3} = \left(\frac{q_1^{m - 1}(1 - p_1^n)}{p_1^{n - 1} + q_1^{m - 1} - p_1^{n - 1}q_1^{m - 1}}\right)\left(\frac{q_2^{m - 1}(1 - p_2^n)}{p_2^{n - 1} + q_2^{m - 1} - p_2^{n - 1}q_2^{m - 1}}\right)
    \end{align*}

    % more application to the fault-tolerance switching problem. Conditioning state of system (X_i) on whether A_1 vs A2 shows up first.

    Now return back to the case from~\exa{brute_force} where $A_1 = (1,0,1,0,\cdots, 1,0)$ with length $2n$ and $A_2 = (1,\cdots,1,0,\cdots,0)$ with length $2m$. For the sake of simplicity, we will also take the symmetric case of $p=q=1/2$. Again define $\Ecal$ to be the event where $A_1$ is observed before $A_2$, and let $P_1 := \Pbb(\Ecal)$. We can again compute $P_1$ by conditioning on the outcomes of trials, but in this case, both $A_1$ and $A_2$ start with $1$. Thus, we instead condition on the outcome of the first two trials $X_1$ and $X_2$. To that end, we denote $\Scal_1$ to be the event that $X_3=1,X_4=0,\cdots=X_{2n-1}=1,X_{2n}=0$ and $\Scal_2$ to be the event that $X_3=\cdots=X_m=1,X_{m+1}=\cdots=X_{2m}=0$. Thus:
    \begin{align*}
        P_1 := \Pbb(\Ecal) &= p\Pbb(\Ecal|X_1=1) + q\Pbb(\Ecal|X_1=0)\\
        &= p\left( p\Pbb(\Ecal|X_1=1,X_2=1) + q\Pbb(\Ecal|X_1=1,X_2=0)\right) + q\Pbb(\Ecal)
    \end{align*}
    where $\Pbb(\Ecal|X_1=0) = \Pbb(\Ecal)$ because neither $A_1$ nor $A_2$ start with $0$.

    Moreover, using the same logic as in the previous problem:
    \begin{align*}
        &\Pbb(\Ecal|X_1=1,X_2=0) = p^{n-1}q^{n-1} + (1 - p^{n-1}q^{n-1})\Pbb(\Ecal|X_1=1,X_2=0,\Scal_1^c)\\
        &= p^{n-1}q^{n-1} + (1 - p^{n-1}q^{n-1})\left[\frac{1}{2}\Pbb(\Ecal|X_1=1,X_2=0,\text{1 flipped to 0}) + \frac{1}{2}\Pbb(\Ecal|X_1=1,X_2=0,\text{0 flipped to 1})\right]\\
        &= p^{n-1}q^{n-1} + (1 - p^{n-1}q^{n-1})\left[\frac{1}{2}\Pbb(\Ecal) + \frac{1}{2}\Pbb(\Ecal|X_1=1,X_2=1)\right]
    \end{align*}
    and
    \begin{align*}
        &\Pbb(\Ecal|X_1=1,X_2=1) = (1 - p^{m-2}q^m)\Pbb(\Ecal|X_1=1,X_2=1,\Scal_2)\\
        &= (1 - p^{m-2}q^m)\left[ \frac{m-2}{2m-2}\Pbb(\Ecal|X_1=1,X_2=1,\text{1 flipped to 0}) + \frac{m}{2m-2}\Pbb(\Ecal|X_1=1,X_2=1,\text{0 flipped to 1})\right]\\
        &= (1 - p^{m-2}q^m)\left[ \frac{m-2}{2m-2}\Pbb(\Ecal|X_1=1,X_2=0) + \frac{m}{2m-2}\Pbb(\Ecal|X_1=1)\right]
    \end{align*}

    Altogether, we obtain a system of three equations with three unknowns. Denoting shorthand notation $P_{1,10} := \Pbb(\Ecal|X_1=1,X_2=0)$ and $P_{1,11} := \Pbb(\Ecal|X_1=1,X_2=1)$, and substituting $p=q=1/2$:
    \begin{align*}
        P_1 &= \frac{1}{2}P_{1,10} + \frac{1}{2}P_{1,11}\\
        P_{1,10} &= \left(\frac{1}{2}\right)^{2n-2} + \frac{1}{2}\left(1 - \left(\frac{1}{2}\right)^{2n-2}\right)(P_1 + P_{1,11})\\
        P_{1,11} &= \left(1 - \left(\frac{1}{2}\right)^{2m-2}\right)\left[\frac{m}{2m-2}P_1 + \frac{m-2}{2m-2}P_{1,10}\right]
    \end{align*}
    Solving the linear system of equations for $n = 5, m = 6$ yields $P_{1,10} = 0.7895$, $P_{1,11} = 0.7884$, and $P_1 = 0.7889$.
\end{example}

The discussion of this simple example segways naturally to more complicated pattern sequences and broader probability distributions of $X_i$, i.e. those that take more than two values. The next theorem provides a result for when there is dependence among the values of $X_i$.

\begin{definition}[Pattern Overlap]
    For a renewal process $X_1, X_2,\cdots$ taking values $x_1, x_2, \cdots$ from a certain probability distribution, we say that a pattern $(x_{(1)}, x_{(2)}, \cdots, x_{(m)})$ has an overlap of size $k < m$ if
    \begin{align*}
        k := \max\{\ell < m | (x_1, \cdots, x_{\ell}) = (x_{m-\ell+1}, \cdots, x_m)\}
    \end{align*}
    That is, $k$ is the largest value such that the first $k$ elements are identical to the last $k$ elements.
    % A pattern $(x_1,\cdots, x_m)$ has overlap of size $k$ if:
    % \begin{align*}
    %     k = \max\{j < m : (x_{m-j+1},\cdots,x_m) = (x_1, \cdots, x_j)\}
    % \end{align*}
    % That is, there exists a size $j$ subsequence of the pattern at the end which matches another size $j$ subsequence of the pattern at the front. 
\end{definition}

\begin{theorem}[Pattern Occurrence for Discrete-State Markov Chain]\label{thm:pattern_occurrence_mc}
    Let $X_1, X_2,\cdots$ denote a sequence of random variables taking values from a discrete-state Markov Chain with transition probability matrix $P := \{P_{ij}\}$ and stationary distribution $\{\pi_k\}$. Let $T$ denote the next time the pattern $(x_1, \cdots, x_m)$ occurs after its first occurrence. 
    % In this problem, we are interested in the expected value of $T$. Within the specific context of the pattern occurrence problem, we refer to a ``renewal'' as the event when the pattern string $(x_1, \cdots, x_m)$ repeats itself. Hence, the interarrival times of such a renewal process are distributed in the same manner as $T$.
    Then:
    \begin{itemize}
        \item When the pattern $(x_1,\cdots,x_m)$ does not contain any overlaps. then the expected time $T$ in between consecutive observations of the pattern is given by
        \begin{align}\label{eq:T_no_overlap_mc}
            \Ebb[T|X_0 = x_0] = \frac{1}{\pi_{x_1}\prod\limits_{i=1}^{m-1} P_{x_i,x_{i+1}}} + \mu(x_0,x_1) - \mu(x_m,x_1)
        \end{align}
        where $\mu(x,y)$ denotes the mean time it takes to reach state $y$ in the Markov chain from state $x$.

        \item When the pattern $(x_1,\cdots,x_m)$ has an overlap $(x_1,\cdots,x_k)$ of size $k$, and $(x_1,\cdots,x_k)$ itself does not contain any overlaps, then the expected time $T$ in between consecutive observations is given by
        \begin{align}\label{eq:T_overlap_mc}
            \Ebb[T|X_0 = x_0] = \frac{1}{\pi_{x_1}\prod\limits_{i=1}^{m-1} P_{x_i,x_{i+1}}} + \frac{1}{\pi_{x_1}\prod\limits_{i=1}^{k-1} P_{x_i,x_{i+1}}} + \mu(x_0,x_1) - \mu(x_m,x_1)
        \end{align}
    \end{itemize}
\end{theorem}

\begin{example}[\thm{pattern_occurrence_mc} for iid Sequence]\label{ex:pattern_occurrence_iid}
    We can specialize the results of~\thm{pattern_occurrence_mc} to the case where the random variables $X_i$ are iid. Let $X_1, X_2,\cdots$ denote a sequence of iid random variables taking on values from a discrete, finite set $\Xcal$. Denote $p_k := \Pbb(X_i= k)$ for all $i$, and let $T$ denote the next time the pattern $(x_1, \cdots, x_m)$ occurs after its first occurrence. Then:
    \begin{itemize}
        \item When the pattern $(x_1,\cdots,x_m)$ does not contain any overlaps. then the expected time $T$ in between consecutive observations of the pattern is given by
        \begin{align}\label{eq:T_no_overlap_iid}
            \Ebb[T] = \frac{1}{\prod\limits_{i=1}^m p_{x_i}}
        \end{align}

        \item When the pattern $(x_1,\cdots,x_m)$ has an overlap $(x_1,\cdots,x_k)$ of size $k$, and $(x_1,\cdots,x_k)$ itself does not contain any overlaps, then the expected time $T$ in between consecutive observations is given by
        \begin{align}\label{eq:T_overlap_iid}
            \Ebb[T] = \frac{1}{\prod\limits_{i=1}^m p_i} + \frac{1}{\prod\limits_{i=1}^{k} p_i}
        \end{align}
    \end{itemize}
\end{example}

Note that, when we return to the motivating example and compute the expected times to obtain, respectively, the $A_1$ and $A_2$ used in~\exa{brute_force}, we obtain the exact same formulas~\eqn{motive_success_time} and~\eqn{motive_failure_time}, derived using brute-force. More specifically, $A_2$ does not have any overlaps, which is why $\Ebb[T_2]$ can be derived using the formula~\eqn{T_no_overlap_iid}; $A_1$ has overlapping patterns in the form of all length-$2j$ subsequences of alternating $(1,0)$, for $1\leq j\leq n-1$, and so $\Ebb[T_1]$ can be derived using the formula~\eqn{T_overlap_iid}.

\begin{remark}
    Some of the standard references in renewal theory~\cite{ross96book,ross06book,ross10book} also provide some discussion on the pattern-occurrence problem from renewal theory, but often only present the iid case of~\exa{pattern_occurrence_iid}. In~\thm{pattern_occurrence_mc}, we extended this result to include a possible dependence structure for its relevance to the specific fault-tolerance and congestion control case studies we investigate later in~\sec{case_studies}. While a rough sketch of the proof for the iid case~\exa{pattern_occurrence_iid} can be found in~\cite{ross96book}, we provide a more detailed derivation of the formulas in our work~\cite{han21book}. The proof to~\thm{pattern_occurrence_mc} can also be found in~\cite{han21book}.
\end{remark}

% The extended version of the problem, which is a problem of interest in more general settings of renewal processes, looks into computing the probability of observing a specific pattern first among a predetermined set of patterns we wish to observe. We investigate the more general problem after addressing this simpler coin tossing problem.
Furthermore, we can address the question of comparing multiple different patterns at once. Let $\{A_1, \cdots, A_M\}$ for $M\in\Nbb^{+}$ be $M$ different patterns of interest, and let $T_{A_i}$ denote the time it takes to observe pattern $A_i$. Denote $T_{\text{min}} := \min\{T_{A_1}, \cdots, T_{A_M}\}$ and denote $P_i$ to be the probability of observing pattern $A_i$ first at time $T_{\text{min}}$. We further denote $T_{A_i|A_j}$ to be the additional time it takes to observe the pattern $A_i$ after $A_j$ has been observed. We are interested in computing the $P_i$ and $\Ebb[T_{\text{min}}]$. 

We further denote $T_{A_i|A_j}$ to be the additional time it takes to observe sequence $A_i$ given that we've already observed $A_j$, for all $i\neq j$. Since all the patterns $\{A_1, \cdots, A_M\}$ are known, both $\Ebb[T_{A_i}]$ and $\Ebb[T_{A_i|A_j}]$ can be computed using either~\thm{pattern_occurrence_mc} or~\exa{pattern_occurrence_iid}. We can then derive a system of equations with these variables as follows:
\begin{align*}
    \Ebb[T_{A_k}] &= \Ebb[T_{\text{min}}] + \Ebb[T_{A_k}-T_{\text{min}}] = \Ebb[T_{\text{min}}] + \sum\limits_{j\neq k}\Ebb[T_{A_k|A_j}]P_j + 0\cdot P_k
\end{align*}
which, combined with the constraint that $P_M := 1 - \sum_{i<M}P_i$ yields $M$ linear equations with $M$ unknowns $P_1, \cdots, P_{M-1}, \Ebb[T_{\text{min}}]$. For the case where $M=2$, we obtain the explicit formula:
\begin{align}\label{eq:min_time_first_prob}
    P_1 &= \frac{\Ebb[T_{A_2}] + \Ebb[T_{A_1|A_2}] - \Ebb[T_{A_1}]}{\Ebb[T_{A_2|A_1}] + \Ebb[T_{A_1|A_2}]},\qquad \Ebb[T_{\text{min}}] = \Ebb[T_{A_2}] - \Ebb[T_{A_2|A_1}]P_1
\end{align}

In relation to~\exa{brute_force}, applying~\eqn{min_time_first_prob} to the case where $A_1$ is $n$ consecutive $1$'s and $A_2$ is $m$ consecutive $0$'s yields the desired result~\eqn{motive_prob}. Likewise, applying~\eqn{min_time_first_prob} to the case where $A_1 := (1,0,\cdots, 1,0)$ and $A_2 := (1,\cdots,1,0,\cdots,0)$ with $n=5,m=6$ implies that $\Ebb[T_{A_1|A_2}] = \Ebb[T_{A_1}]$ and $\Ebb[T_{A_2|A_1}] = \Ebb[T_{A_2}]$. With $p=q=1/2$, we obtain the numerical values derived at the end of~\exa{brute_force}.

\begin{remark}[Alternative Pattern-Occurrence Problem with Random Walks]
    If we are interested in keeping track of longer pattern sequences of impulsive disturbances, the pattern-occurrence problem can also be solved using an alternative approach with random walks. Borrowing influence from common motivational problems such as the Gambler's Ruin problem, the theory of random walks can be used to determine the expected time it takes the system to reach certain boundaries imposed on the system state, upon which the modulation control mechanism takes over. For the sake of keeping this paper focused, we defer discussion of the connections between the pattern-occurrence problem and the theory of random walks to~\cite{han21book}. A comprehensive treatment of random walk theory background needed to understand these connections can also be found in~\cite{han21book}.
\end{remark}

